Learning Patient-Specific Disease Dynamics with Latent Flow Matching for Longitudinal Imaging Generation

Understanding disease progression is a central clinical challenge with direct implications for early diagnosis and personalized treatment. While recent generative approaches have attempted to model progression, key mismatches remain: disease dynamics are inherently continuous and monotonic, yet latent representations are often scattered, lacking semantic structure, and diffusion-based models disrupt continuity with random denoising process. In this work, we propose to treat the disease dynamic as a velocity field and leverage Flow Matching (FM) to align the temporal evolution of patient data. Unlike prior methods, it captures the intrinsic dynamic of disease, making the progression more interpretable. However, a key challenge remains: in latent space, Auto-Encoders (AEs) do not guarantee alignment across patients or correlation with clinical-severity indicators (e.g., age and disease conditions). To address this, we propose to learn patient-specific latent alignment, which enforces patient trajectories to lie along a specific axis, with magnitude increasing monotonically with disease severity. This leads to a consistent and semantically meaningful latent space. Together, we present $\Delta$-LFM, a framework for modeling patient-specific latent progression with flow matching. Across three longitudinal MRI benchmarks, $\Delta$-LFM demonstrates strong empirical performance and, more importantly, offers a new framework for interpreting and visualizing disease dynamics.

==> sec/ControlNet_Pre.tex <==

\subsection{Preliminaries }
\label{sec:preliminaries} 



A Latent Diffusion Model (LDM)~\cite{rombach2022high} is a deep generative paradigm that extends the Denoising Diffusion Probabilistic Model (DDPM)~\cite{ho2020denoising}. Instead of directly perturbing the image $\mathbf{x}$, an LDM perturbs the latent representation $\mathbf{z}_0$, which is obtained using a pre-trained encoder $E$, such that $\mathbf{z}_0 = E(\mathbf{x})$. A corresponding decoder $D$ can then reconstruct the original image via $\mathbf{x} = D(\mathbf{z}_0)$.


%% -----------

Assume a Markov process panning $T$ discrete timesteps that incrementally adds noise to the latent variable. As $ t $ approaches $ T $, the latent representation  converges to an isotropic Gaussian distribution:
\begin{equation}
\mathbf{z}_0 \rightarrow \mathbf{z}_1 \rightarrow \cdots \rightarrow \mathbf{z}_T \sim \mathcal{N}(\mathbf0, \mathbf I), \quad
q(\mathbf{z}_t \mid \mathbf{z}_{t-1}) = \mathcal{N}(\mathbf{z}_t; \sqrt{1 - \beta_t} \mathbf{z}_{t-1}, \beta_t \mathbf{I}),
\end{equation}
where $ \beta_t $ follows a predefined variance schedule.  The LDM learns to reverse this stochastic process and is parameterized by a neural network  \( \boldsymbol{\epsilon}_\theta \), which maximize the posterior probability at each step:
\begin{equation}
p_\theta(\mathbf{z}_{t-1} \mid \mathbf{z}_t) = \mathcal{N}(\mathbf{z}_{t-1}; \mu_\theta(\mathbf{z}_t, t), \Sigma_\theta(t)). 
\end{equation}
The training objective~\cite{ho2020denoising} is reparameterized to directly predict the noise component $\boldsymbol{\epsilon}$ at each step, with the network output $\boldsymbol{\epsilon}_\theta(\mathbf{z}_t, t) \approx \boldsymbol{\epsilon}$ optimized using a mean squared error (MSE) loss, ensuring alignment with the true noise perturbation.
\begin{equation}
\mathcal{L}_{\epsilon}  \coloneqq  \mathbb{E}_{t, \mathbf{z}_0, \boldsymbol{\epsilon} \sim \mathcal{N}(0, I)} \left[ \|\boldsymbol{\epsilon} - \boldsymbol{\epsilon}_\theta(\mathbf{z}_t, t) \|^2 \right]
\end{equation}


ControlNet~\cite{zhang2023adding} extends LDMs by introducing covariates $\mathbf{c}$ and a parallel trainable network that transforms the conditioning input via $\mathbf{f}_c = \mathcal{T}_\psi(\mathbf{c})$. This modifies the reverse denoising process as $\mathbf{h}' = \mathbf{h} + \lambda \mathbf{f}_c$, where $\mathbf{h}$ is the hidden feature map and $\lambda$ controls the influence of $\mathbf{c}$. The resulting conditioned loss function is defined as: 
\begin{equation}
\mathcal{L}_{\epsilon} \coloneqq \mathbb{E}_{t, \textbf{z}_0, \boldsymbol{\epsilon} \sim \mathcal{N}(0, I)} \left[ 
\lVert \boldsymbol{\epsilon} - \boldsymbol{\epsilon}_\theta(\textbf{z}_t, \textbf{c}, t) \rVert^2 \right].
\end{equation}



% To incorporate the condition,  ControlNet incorporates a parallel trainable network, enable high-quality image synthesis. 
% ControlNet incorporates a parallel trainable network that learns a transformation of the conditioning input $ f_c = \mathcal{T}_\psi (c)$, where $\mathcal{T}_\psi$ is a trainable function parameterized by $\psi$, mapping the conditioning input $c$ to a feature space. This transformed conditional feature is then used to modify the  reverse denoising process, with  $\mathbf  h' = \mathbf  h + \lambda \mathbf f_c$,  $h$ is the hidden feature map from denoising network, $\lambda$ is a scaling factor controlling how much $c$ influences $h$. 



% ---------------------------------
    \calvin{Rewrite till here...}
% ---------------------------------



==> sec/method_save.tex <==


\section{Methodology}
\label{sec:method}



\subsection{Preliminaries }
\label{sec:preliminaries} 


A Latent Diffusion Models (LDMs)~\cite{rombach2022high} is a deep generative paradigm extends the  Denoising Diffusion Probabilistic Model (DDPM)~\cite{ho2020denoising} by shifting the diffusion process from pixel space to a more compact latent space. Instead of directly perturbing the image $x$, LDM first derive latent $z_0$ via a pre-trained autoencoder composed of an encoder $\mathcal{E}$ and a decoder $\mathcal{D}$, such that the encoder maps the input sample $x$ to the latent space $z_0 = \mathcal{E}(x),$ while the decoder  reconstructs the original image via $x = \mathcal{D}(z_0)$.  



LDMs learn to reverse a Markov process panning $T$ discrete timesteps that incrementally adds noise to a latent, As $ t $ approaches $ T $, the latent representation asymptotically converges to an isotropic Gaussian distribution:
\[
\mathbf{z}_0 \rightarrow \mathbf{z}_1 \rightarrow \cdots \rightarrow \mathbf{z}_T \sim \mathcal{N}(0, I), \quad
q(\mathbf{z}_t \mid \mathbf{z}_{t-1}) = \mathcal{N}(\mathbf{z}_t; \sqrt{1 - \beta_t} \mathbf{z}_{t-1}, \beta_t \mathbf{I})
\]
, where $ \beta_t $ follows a predefined variance schedule.  The \textit{reverse diffusion process} seeks to invert this stochastic transformation, gradually refining $ z_T $ back into a coherent latent representation $ z_0 $. is parameterized with a neural network \( \boldsymbol{\epsilon}_\theta \) to estimate the noise:
\[
p_\theta(\mathbf{z}_{t-1} \mid \mathbf{z}_t) = \mathcal{N}(\mathbf{z}_{t-1}; \mu_\theta(\mathbf{z}_t, t), \Sigma_\theta(t))
\]



Following~\cite{ho2020denoising}, the training objective is achieved by reparameterized in terms of associated noise component $, \epsilon $, enabling the denoising network to directly predict the noise contamination $ \boldsymbol{\epsilon} _\theta(z_t, t) \approx  \boldsymbol{\epsilon} $ with mean squared error (MSE) loss nsuring that the predicted noise aligns with the true noise perturbation:
\[
\mathcal{L}_{\epsilon}  \coloneqq  \mathbb{E}_{t, \mathbf{z}_0, \boldsymbol{\epsilon} \sim \mathcal{N}(0, I)} \left[ \|\boldsymbol{\epsilon} - \boldsymbol{\epsilon}_\theta(\mathbf{z}_t, t) \|^2 \right]
\]

ControlNet~\cite{zhang2023adding} extends LDMs by introducing covariates $c$ and conditioning mechanisms that guide the diffusion denoising process. To incorporate the condition,  ControlNet incorporates a parallel trainable network, enable high-quality image synthesis. 
ControlNet incorporates a parallel trainable network that learns a transformation of the conditioning input $ f_c = \mathcal{T}_\psi (c)$, where $\mathcal{T}_\psi$ is a trainable function parameterized by $\psi$, mapping the conditioning input $c$ to a feature space. This transformed conditional feature is then used to modify the  reverse denoising process, with  $\mathbf  h' = \mathbf  h + \lambda \mathbf f_c$,  $h$ is the hidden feature map from denoising network, $\lambda$ is a scaling factor controlling how much $c$ influences $h$. 

 The modified reverse process incorporates this conditioning input into the noise prediction function $\boldsymbol \epsilon_\theta(\textbf z_t, t, \textbf c) \approx \boldsymbol \epsilon$, resulting in the following new conditioned loss function:
\begin{equation}
\mathcal{L}_{\epsilon} \coloneqq \mathbb{E}_{t, \textbf{z}_0, \boldsymbol{\epsilon} \sim \mathcal{N}(0, I)} \left[ 
\lVert \boldsymbol{\epsilon} - \boldsymbol{\epsilon}_\theta(\textbf{z}_t, t, \textbf{c}) \rVert^2 \right].
\end{equation}







We address this with a dual-control approach using imaging features and patient-specific geometry. Ensuring temporal consistency requires imaging features that maintain fidelity across time points. A major limitation of existing methods is their failure to preserve individual anatomical structures, which is essential for meaningful disease progression modeling. Without maintaining patient-specific geometry, even high-resolution generated images may lack clinical relevance and fail to provide useful diagnostic insights. 


% By integrating both visual similarity constraints and structural consistency mechanisms, our method generates realistic, patient-specific disease progression, ensuring both image quality and medical accuracy.

% -----------------------
\subsection{Method Overview}

While LDMs achieve high-fidelity synthesis and ControlNet enables guided generation, a critical question persists: \textit{How can we synthesise patient-specific, anatomically coherent disease progression over time?}   Insufficient infromed may produce anatomically implausible outputs that violate realistic brain morphology.
This paper answers by grounding generation in modelling anatomical geometry and disease trajectory. Figure \ref{} illustrates the overall design. Starting from a patient’s baseline 3D imaging (time $t$), with assigned time duration between the future time point $t+d$, we have totally four conditions with two specific at current time point indicates the input latent and patient attributes at time $t$: $\mathbf z_t$ and $\mathbf  c_t$, and two new conditions \ourgraph~and \ourfeature~which is feature at $t+d$: $\mathbf g_{t+d}$ and $\mathbf f_{t+d}$.
The $\mathbf z_t$ is the latent derived from the image at time point $t$ with $\mathcal E(\cdot)$, and the $\mathbf c_t$ is
patient demographics and disease related condtion (\eg cognitive scores and brain region size in AD). 


% Incorporate Clinical Endpoints in Embedding: We can inject the cognitive diagnosis label or a cognitive score into the embedding training. For example, use a supervised contrastive loss where not only same patient = positive pair, but also perhaps enforce that patients with similar diagnoses cluster somewhat. Alternatively, add an auxiliary classifier on the embedding to predict diagnosis (CN/MCI/AD)



% dvanced atrophy in the same time span.



Our  first propose condition is \ourgraph~with a brain segmentation is converted into the baseline $\mathbf g_t$ where each anatomical region is a node, and edges represent structural correlations (e.g. regions that atrophy together) 
with pretrained morph function $\Phi(\cdot)$ to morph into the predicted $\mathbf  g_{t+d}$. the model explicitly accounts for structural anatomy,  graph constraint helps preserve the spatial relationships between regions. The second feature is the longitudinal patient specific-feature $\mathbf f_{t+d}$  sampled start from input $\mathbf f_t$ and given duration $d$, which is further elaborated in Sec. $ \ref{sec:anagraph} $ and Sec.$\ref{sec:arcrank}$, respectively. The subsections that follow introduce our conditioning features and explain how they are incorporated to steer the generative process with clinical relevance and structural consistency.



% Finally
Given a diffusion denoiser decoder state $\mathbf{h}$, we formulate the conditional generation consider transformation of $\mathbf{h}$ via a generalized AdaLN~\cite{} mechanism: 
\begin{equation}
\begin{aligned}
[\boldsymbol{\alpha}_a,\, \boldsymbol{\beta}_a,\, \boldsymbol\gamma_a,\,
 \boldsymbol{\alpha}_p,\, \boldsymbol{\beta}_p,\, \boldsymbol\gamma_p] 
&= \mathrm{MLP}\left([\mathbf{z}_0,\, \mathbf{c}_t,\, \mathbf{f}_{t+d}]\right) \\
\mathbf{h}' 
&= \mathbf{h} + \boldsymbol\gamma_a \cdot \mathrm{Attn}\left(
    \boldsymbol{\alpha}_a \odot \mathrm{LN}(\mathbf{h}) + \boldsymbol{\beta}_a,\ 
    \mathbf{g}_{t+d}
\right) \\
\mathbf{h}'' 
&= \mathbf{h}' + \boldsymbol\gamma_p \cdot \mathrm{MLP}\left(
    \boldsymbol{\alpha}_p \odot \mathrm{LN}(\mathbf{h}') + \boldsymbol{\beta}_p
\right)
\end{aligned}
\end{equation}

Here, the $\mathrm{MLP}(\cdot)$ receives a concatenation of the latent vector $\mathbf{z}_0$, the context vector $\mathbf{c}_t$, and future-aware features $\mathbf{f}_{t+d}$, and produces two sets of modulation parameters: $(\boldsymbol{\alpha}_a, \boldsymbol{\beta}_a, \boldsymbol{\gamma}_a)$ for attention and $(\boldsymbol{\alpha}_p, \boldsymbol{\beta}_p, \boldsymbol{\gamma}_p)$ for feedforward transformation. 
These parameters adaptively scale and shift the layer normalized hidden state ($\mathrm{LN}(\mathbf{h})$) through multiplicative operation ($\odot$), enabling flexible control of the denoising process conditioned on patient context. 
The attention module $\mathrm{Attn}(\cdot)$ queries future-guided representations $\mathbf{g}_{t+d}$ to inform updates, and the final output $\mathbf{h}''$ integrates both contextual and temporal information in a modulated residual path.


 The modified reverse process incorporates this conditioning input into the renewed noise prediction function $\boldsymbol \epsilon_\theta(\textbf z_t, t, \textbf c) \approx \boldsymbol \epsilon$, resulting in the following new conditioned loss function:
\begin{equation}
\mathcal{L}_{\epsilon} \coloneqq \mathbb{E}_{t, \textbf{z}_0, \boldsymbol{\epsilon} \sim \mathcal{N}(0, I)} \left[ 
\lVert \boldsymbol{\epsilon} - \boldsymbol{\epsilon}_\theta(\textbf{z}_t, \tau, t, \mathbf{c}_t, d, \mathbf{f}_{t+d}, \mathbf{g}_{t+d}) \rVert^2 \right].
\end{equation}
% \, 



$\tau \in \{0, 1, 2, \dots, T\}$


% ---------------------------------
    \calvin{Rewrite till here...}
% ---------------------------------


% is obtained using SynthSeg from Free Surfer~\cite{}



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{asset//img/image.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}



Similar to Litrici \etal~\cite{litrico2024tadm}, we encode the given query time $t$ and the futuer time $t+\Delta t$ via a positional time embedding sinusoidal positional encoding. In our design, we use Vision Transformer (ViT) architecture for Diffusion denoiser and the ControlNet.






\subsection{ArcRank: Longitudinal Contrastive Alignment of Anatomy}
\label{sec:arcrank}
In longitudinal data, each subject’s scans form a trajectory of change.  
We wanna enforce the learning of patient-specific disease progression trcjectory in latent space. Most contrastive loss in afore-mentioned caseds pull similar image together, ie put same imaging from same patient together interchangeably close, without indicating which is earlier., or pulls adjacent timepoints together, but we might also want to encode directionality (i.e. understanding that one comes before the other linewise), to better sample it when inference new future latent.
The latent mitigates the risk that the generative model produces a future scan resembling a different patient. 

Inspired by ArcFace Loss, that propose to pull the angle from same group similar. We propose \ourfeature, which consistitude two parts, the firts align different timepoint along with the same angle line, effectively learning an identity vector that captures stable person-specific attribute. The second to make it chronicolly meaning, we propose the ranking part that is pull，  time-aware loss further arranges the latent space so that time progression is encoded smoothly， scans that are close timepoint, end up close in representation，  whereas scans longer apart diverge.


This is conceptually similar to Longitudinal Neighborhood Embedding (LNE) approaches~\cite{ouyang2022self}
propose a smooth trajectory field where each trajectory captures changes in brain ages between a pair of MRIs extracted from a longitudinal sequence. Our method is also learn a vector field that in each patient aligns with same angle (direction), but the magnitude is varies according to the state， modulate its output based on “how far along” the patient’s trajectory is, leading to more accurate progression trends.



A patient with temporally ordered image features $\mathbf{f}_i,\mathbf{f}_j$ at times $t_i < t_j$, we define the ArcRank loss by combining an angular alignment term with a norm-ranking term:

\[
\mathcal{L}_{\text{ArcRank}} = \sum_{\substack{i<j\\ \text{same patient}}}
\left[ \angle(\mathbf{f}_i, \mathbf{f}_j) + \lambda\, \max\left(0,\,\|\mathbf{f}_i\| + m - \|\mathbf{f}_j\|\right) \right],
\]

where
\[
\angle(\mathbf{f}_i, \mathbf{f}_j) = \arccos\left(\frac{\mathbf{f}_i \cdot \mathbf{f}_j}{\|\mathbf{f}_i\| \|\mathbf{f}_j\|}\right)
\]
is the angular (geodesic) distance between feature vectors. Here, $\lambda > 0$ balances the two terms, and $m > 0$ is a margin that enforces strict norm ordering.



\paragraph{Angular Term:} The angle term $\angle(\mathbf{f}_i, \mathbf{f}_j)$ encourages same-patient features to align directionally on the unit hypersphere. This is analogous to contrastive self-supervised learning approaches that optimize cosine similarity. See: 

On the Importance of Embedding Norms in Self-Supervised Learning, and angular-margin methods like  AMC-Loss.



\paragraph{Rank Term:} The hinge loss $\max(0, \|\mathbf{f}_i\| + m - \|\mathbf{f}_j\|)$ ensures that feature norms increase with time: later-time features must have strictly greater norm than earlier ones. This leverages the fact that embedding norm magnitudes often correlate with semantic richness or confidence.

% Magnitude Ranking Across Timepoints, 
\begin{itemize}
    \item $\lambda$: trade-off between angular and chronological alignment.
    \item $m$: margin to ensure meaningful norm separation.
\end{itemize}


Minimizing $\mathcal{L}_{\text{ArcRank}}$ aligns same-patient features angularly while enforcing temporal ordering through vector norm ranking. The loss is fully self-supervised, relying only on patient identity and the intrinsic order of timestamps.



\paragraph{Scaling Function Term:} 
$$
\mathbf{f}_{t+\Delta t} = \gamma_t \cdot \mathbf{f}_t
$$

Where $\gamma\_t$ is a scalar field (same spatial shape as $\mathbf{f}\_t$), predicting how much to scale the magnitude at each point.

Then, train a network to predict $\gamma\_t$ given:

 $\mathbf{f}\_t$
 optionally, an image or anatomical context at $t$ or $t+\Delta t$

 Loss Function to Supervise $\gamma\_t$

If you have ground truth $\mathbf{f}\_{t+\Delta t}$, then supervise:

$$
\mathcal{L}_{\text{scale}} = \left\| \gamma_t \cdot \mathbf{f}_t - \mathbf{f}_{t+\Delta t} \right\|^2
$$

If only magnitudes are known:

$$
\mathcal{L}_{\text{mag}} = \left\| \gamma_t \cdot \|\mathbf{f}_t\| - \|\mathbf{f}_{t+\Delta t}\| \right\|^2
$$



   % In effect, this tackles the problem of patient heterogeneity: two patients with different baseline embeddings will produce different future outcomes, aligning with individualized disease paths rather than an average trajectory.



% Controllable Consistency in Image or Video
% Generation via Reference Feature Guidance









% -----------------------
\subsection{AnaGraph: Representing Masks as Graph Nodes}
\label{sec:anagraph}


We propose AnaGraph, a graph-based representation that models anatomical structures in medical images. Each node corresponds to a segmented region, forming a graph that captures spatial relationships at baseline. The goal, however, is to predict anatomy at a future time point. A static graph provides limited information about how anatomy evolves. To address this, we introduce a morph function $M(\cdot)$ that deforms the baseline graph toward the future anatomy. This warped baseline segmentation acts as a proxy for future anatomy, offering directional cues to enable temporally informed predictions. 



Given an image $x$ with its corresponding segmentation map $s$, we construct a graph representation $G = (\mathcal V, \mathcal E)$, where $V = \{ v_i \}_{i=1}^{N}$ denotes the set of $N$ segmented regions, $E = \{ e_{ij} \mid d(v_i, v_j) \leq \tau \}$ represents the edges based on spatial proximity $d(v_i, v_j)$ with a distance threshold $\tau$. We denote the graph construction process as $\mathcal{G}=G(x, s, a)$ from $x$ and patients attributes from notes $a$. These features can be viewed as a set of unordered nodes which are denoted as $\mathcal{V}=\{v_1,v_2,\cdots,v_N\}$.  We employ the Vision Graph (ViG)~\cite{han2022vision} to propagate information across segmented regions and encode their relationships within a latent space.


% the diffusion model and 

We aim to predict future anatomical segmentations using a graph-based model supervised by Dice loss. At time $t$, we initialise an anatomical graph $\mathbf{g}_t$ with node features from segmentation masks $\{s_{t,1}, s_{t,2}, \dots, s_{t,n}\} \sim \mathcal{S}$.

To model temporal change, we apply a morph function $M(\cdot)$ implemented via a Vision Graph (ViG)~\cite{}, which follows a ViT-style encoder-decoder. The predicted future mask $M(\mathbf{g}_t)$ is trained against the ground truth $s_{t+\Delta t}$ using:

\[
\mathcal{L}_{\text{dice}} = 1 - \text{Dice}(M(\mathbf{g}_t), \mathbf{g}_{t+\Delta t})
\]
The goal is to learn meaningful  embeddings that preserve the biological geometric structure  while encoding region-wise interactions. This learned middle representation is then used as a conditioning feature for the diffusion model.



\paragraph{\ourgraph~guided Control Process}
After pretraining \ourgraph, we integrate it into the ControlNet framework. Specifically, we use the encoder $M_{\small E}$ to extract anatomical features, which are injected into each layer of ControlNet as conditional input. The encoder remains trainable to adapt its representations to the control task.



% The above graph-level processing can be denoted as $X'=\text{GraphConv}(X)$. 


\begin{figure}[t]%[htpb]
  % \hspace{-0.2pt}
  \centering
  \includegraphics[width=1.02 \linewidth ]{asset/img/ssl.jpg}   % trim=5 110 20 10,clip
  \hspace{-0.3cm}
   \caption{Contrastive Longitudinal Alignment Prior.}
  \label{fig:clap}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{asset//img/arch.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}







% ---------------------------------
    \calvin{Rewrite till here...}
% ---------------------------------


















==> sec/prepare.tex <==


4. Pipeline Enhancements and Missing Components

Beyond the core model, a few additional enhancements could strengthen the overall pipeline:

    Multi-Task Learning with Clinical Outcomes: As hinted in the gaps, integrating a clinical prediction task can add value. For instance, alongside generating the future MRI, have the model (or a linked sub-network) predict the patient’s cognitive score or conversion probability at that future time. This could be done by feeding the generated MRI (or its embedding) into a classifier/regressor. During training, we have ground-truth future diagnoses/scores, so we can train the model to minimize error in that prediction too. This multi-task setup would bias the image generation to not just look plausible, but also to contain relevant disease markers that drive the correct clinical label. For example, if the model tries to predict that the patient will convert to AD in 2 years, the generated 2-year MRI should show AD-like atrophy patterns to support that prediction. By aligning image generation with clinical labels, we ensure the synthetic images are not just realistic-looking but also reflect the underlying pathology progression. This can be a compelling addition in a paper: “Our method not only generates future MRIs but also predicts clinical progression, achieving X\% accuracy in identifying converters vs non-converters, outperforming Y.” It demonstrates the practical utility of the approach for prognosis.

    Uncertainty Quantification: Incorporating an estimate of uncertainty in predictions is valuable, as disease progression is stochastic. BrLP introduced the Latent Average Stabilization (LAS) to derive a measure of uncertainty by sampling multiple predictions and measuring their variability. We can adopt a similar concept. For example, run the diffusion model $n$ times with slight perturbations (or different noise seeds) to generate an ensemble of future MRIs for the same input. Then compute statistics on the predicted anatomical changes (e.g. variance in ventricle volume across samples). A high variance might indicate uncertainty in that patient’s trajectory. During inference, the model could output not just a single MRI but an interval or confidence (e.g. “hippocampal volume will decrease by 5–10\% with 90\% confidence”). Technically, diffusion models naturally allow drawing many samples, so we leverage that. To integrate into training, one could even encourage the model to estimate its own uncertainty – perhaps a secondary network that reads the latent and predicts a scalar uncertainty, trained by how consistent multiple samples are. While not necessary for the method to function, having an uncertainty metric can elevate a publication by addressing reliability (e.g. giving clinicians a sense of confidence in the prediction). It also helps when a patient’s outcome is inherently hard to predict (the model can signal “low confidence”).

    External Validation and Domain Adaptation: Ensure the method is tested beyond ADNI, or at least mention the plan for it. Since the question focuses on method, this might be beyond scope, but for a cohesive story: emphasize that the approach is generalizable to other longitudinal neuroimaging cohorts. We might mention that training on multi-site data (ADNI plus others, like AIBL, OASIS etc. as BrLP did
    ) is possible thanks to the latent diffusion’s robustness, and that the model can handle variability in scans. Possibly propose using augmentation (intensity, noise, slight affine transforms) to make the model more robust to input variations. Also, if needed, a fine-tuning scheme could adapt the model to a new dataset by updating the patient embedding network while freezing the diffusion part, etc.

    Visualization of Learned Progression: To strengthen the paper narrative, consider visualizing what the model learns. For example, plot the patient embedding trajectory for a few subjects (embedding projected to 2D or along principal components) to show that it moves monotonically over time and separates different progression rates. Or visualize the effect of time conditioning: take one baseline MRI and generate outputs at 3, 6, 12, 24 months – show these in a figure to illustrate the progression. Additionally, if using segmentation mask guidance, show an example of baseline mask vs predicted future mask vs real future mask, demonstrating the method’s anatomical foresight. Such visual evidence will make the story more convincing that the method captures the disease dynamics.




\section{Methodology}

% TODO Important
% This transformed conditional feature is then used to modify the  reverse denoising process. One approach is  residual feature injection, where the conditioning signal is processed in a separate path and injected into the denoising network using residual connections $h' = h + \lambda f_c$, where $h$ is the hidden feature map from denoising network, $\lambda$ is a scaling factor controlling how much $c$ influences $h$.  However, this method provides soft conditioning, allowing a high degree of freedom. In some cases, it is necessary to apply localized and more refined control.  
% Thus, another approach to control is through cross-attention mechanisms, which dynamically adjust the importance of different regions in the  feature maps based on the control feature, rather than simply adding it as a residual connection. The modified attention function is defined as:  
% \begin{equation}
% \text{Attention}(Q, K, V) = \text{softmax} \left( \frac{Q K^T}{\sqrt{d}} \right) V, 
% \end{equation}  
% where the query \( Q = W_Q \cdot h \) comes from the latent feature of the denoising network, while the key \( K = W_K \cdot f_c \) and value \( V = W_V \cdot f_c \) are derived from the control feature.








\subsection{Old Version of Method}
Our primary objective is to generate authentic medical image for disease progression prediction and diagnosis. To achieve this, we identify the key challenges in two-fold: First, disease diagnosis is patient-wise that require the generated image authentically present patient body part 
in a truthful way regardless to pathotoligical changes. Second, it should authentical present the longitudinal information, i.e., the disease progression information in medical image. 







% To address the problem of generaing authentic medical image, we first 


% Our goal is to develop a framework that can generate 
% high fedality logitudical medical image in a geometry-sensitive way to improve diagnosis quality.
To achieve this, we propose to the \textit{Anatomical Geometry-Retrieval Graph}, which mapping anatomical structure and functional topography within the given image, and use it to guide the generation of future longitudinal image, as a way for injection meaningful prior 



 Specifically, we propose Contrastive Longitudial Alignment Pre-training (CLAP) for self-supervised graph generation (see Sec. \ref{sec:clap}), which will then serve as guidance signals provided to the
image generation process using diffusion model (see Sec. \ref{sec:generation}). 

In the following sections, we will delve into the key technical designs that enable its functionality.





% \subsection{Proposed Pipeline - Brain Latent Progression (BrLP)}
% We now introduce the architecture of BrLP, comprising four key components: an LDM, a ControlNet, an auxiliary model, and a LAS block, each described in successive paragraphs. These four components, summarized in Figure~\ref{fig:pipeline}, collectively address the challenges outlined in the introduction. In particular, the LDM is designed to generate random 3D brain MRIs that conform to specific covariates, while ControlNet aims to specialize these MRI scans to specific anatomical structures of a subject. Additionally, the auxiliary model leverages prior knowledge of disease progression to improve the precision in predicting the volumetric changes of specific brain regions. Finally, the LAS block is used during inference to improve spatiotemporal consistency. Details concerning the training process and hyperparameter settings are provided in Table 1 of the Supplementary Material.

\subsubsection{LDM - Learning the brain MRIs distribution.}
Building upon~\cite{pinaya2022brain}, we train an LDM aimed to generate 3D brain MRIs mirroring specific covariates $c = \langle s, v \rangle$, where $s$ includes subject-specific metadata (age, sex, and cognitive status) while $v$ encompasses progression-related metrics such as volumes of brain regions (hippocampus, cerebral cortex, amygdala, cerebral white matter, and lateral ventricles) linked to AD progression~\cite{pini2016brain}. The construction of the LDM is a two-phase process. Initially, we train an autoencoder $(\mathcal{E}, \mathcal{D})$ (block A in Figure~\ref{fig:pipeline}) designed to produce a latent representation $z = \mathcal{E}(x)$ for each brain MRI $x$ within our dataset. Subsequently, we train a conditional UNet (block B in Figure~\ref{fig:pipeline}), represented as $\epsilon_\theta$, with network parameters $\theta$, aimed to estimate the noise $\epsilon_\theta(z_t, t, c)$ necessary for reverting from $z_t$ to $z_{t-1}$, as mentioned in Section \ref{sec:background}. We train $\epsilon_\theta$ by minimizing the loss $\mathcal{L}_{\epsilon}$ (Eq.~\ref{eqn:ddpmloss}). Covariates $c$ are integrated into the network as conditions using a cross-attention mechanism, in line with~\cite{rombach2022high}. The generation process initiates by sampling random Gaussian noise $z_T \sim \mathcal{N}(0,I)$ and then iteratively reverses each diffusion step $z_t \to z_{t-1}$ for $t=T, \dots, 1$. Decoding the output $z_0$ from the final step $t=1$ yields a synthetic brain MRI $\hat x = \mathcal{D}(z_0)$ that follows the specified covariates $c$.



\subsubsection{Proposed auxiliary model - Leveraging disease prior knowledge.}
\label{sec:auxiliarymodel}
AD-related regions shrink or expand over time and at different rates~\cite{pini2016brain}. Deep-learning-based spatiotemporal models strive to learn these progression rates directly from brain MRIs in a black-box manner, which can be very challenging. To aid this process, we propose incorporating prior knowledge of volumetric changes directly into our pipeline. To do so, we exploit an auxiliary model $f_\psi$ (block D in Figure~\ref{fig:pipeline}) able to predict how the volumes of AD-related regions change over time and provide this information to the LDM via the progression-related covariates $v$. The choice of our auxiliary model is tailored to two scenarios, making BrLP flexible for both cross-sectional and longitudinal data. For subjects with a single scan available at age $A$, we employ a regression model to estimate volumetric changes $\hat{v}^{(B)} = f_\psi(c^{(A)})$ at age $B$. For subjects with $n$ past visits accessible at ages $A_1, \dots, A_n$, we predict $\hat{v}^{(B)} = f\psi(c^{(A_1)}, \dots, c^{(A_n)})$ using Disease Course Mapping (DCM)~\cite{schiratti2017bayesian,koval2021ad}, a model specifically designed for disease progression. DCM is intended to provide a more accurate trajectory in alignment with the subject's history of volumetric changes available. While we employ DCM as a potential solution, any suitable disease progression model can be used in BrLP.


\subsubsection{Inference process.}
Let $x^{(A)}$ be the input brain MRI from a subject at age $A$, with known subject-specific metadata $s^{(A)}$ and progression-related volumes $v^{(A)}$ measured from $x^{(A)}$. As summarized in block E from Figure~\ref{fig:pipeline}, to infer the brain MRI $x^{(B)}$ at age $B > A$, we perform six steps: i) predict the progression-related volumes $\hat v^{(B)} = f_\psi(c^{(A)})$ using the auxiliary model; ii) concatenate this information with the subject-specific metadata $s^{(B)}$ to form the target covariates $c^{(B)} = \langle s^{(B)}, \hat v^{(B)}\rangle$; iii) compute the latent $z^{(A)} = \mathcal{E}(x^{(A)})$; iv) sample random Gaussian noise $z_T \sim \mathcal{N}(0,I)$; v) run the reverse diffusion process by predicting the noise $\epsilon_{\theta, \phi}(z_t, t, c^{(B)}, z^{(A)})$ to reverse each diffusion step for $t=T,\dots,1$; and finally vi) employ the decoder $\mathcal{D}$ to reconstruct the predicted brain MRI $\hat{x}^{(B)} = \mathcal{D}(z_0)$ in the imaging domain. This inference process is summarized into a compact notation $\hat z^{(B)} = \mathcal{I}(z_T, x^{(A)}, c^{(A)})$ and $\hat x^{(B)} = \mathcal{D}(\hat z^{(B)})$.


\subsubsection{Enhance inference via proposed Latent Average Stabilization (LAS).}
Variations in the initial value $x_T \sim \mathcal{N}(0,I)$ can lead to slight discrepancies in the results produced by the inference process. These discrepancies are especially noticeable when making predictions over successive timesteps, manifesting as irregular patterns or non-smooth transitions of progression. Therefore, we introduce LAS (block F in Figure~\ref{fig:pipeline}), a technique to improve spatiotemporal consistency by averaging different results of the inference process. In particular, LAS is based on the assumption that the predictions $\hat z^{(B)} = \mathcal{I}(z_T, x^{(A)}, c^{(A)})$ deviate from a theoretical mean $\mu^{(B)} = \mathbb{E}[\hat z^{(B)}]$. To estimate the expected value $\mu^{(B)}$, we propose to repeat the inference process $m$ times and average the results:
\begin{equation}
\mu^{(B)} =  \mathop{\mathbb{E}}_{z_T \sim \mathcal{N}(0,I)} \bigg[ \mathcal{I}(z_T, x^{(A)}, c^{(A)})\bigg] \approx \frac{1}{m}\sum^m \mathcal{I}(z_T, x^{(A)}, c^{(A)}).
\end{equation}
Similar to before, we decode the predicted scan as $\hat x^{(B)} = \mathcal{D}(\mu^{(B)})$. The entire inference process (with $m=4$) requires $\sim$4.8s per MRI on a consumer GPU.





% A stack of Grapher module and FFN module constitutes the ViG block which serves as the basic building unit for constructing a network. Based on the graph representation of images and the proposed ViG block, we can build the ViG network for visual tasks as shown in Figure~\ref{Fig:vig}. Compared to vanilla ResGCN~\cite{deepgcn}, our ViG can maintain the feature diversity (Figure~\ref{Fig:diversity}) as the layer goes deeper so as to learn discriminative representations.


% , and $F = \{ f_i \}_{i=1}^{N}$ is the node feature set, encoding the corresponding biological features 

% composition of parts (\eg, a human can be roughly divided into head, upper body, arms and legs), and graph structure can construct the connections among those parts; 4) the advanced research on GNN can be transferred to address visual tasks.




% \begin{equation}
% f_c = \mathcal{T}_\psi(G),
% \end{equation}

% which is then used to condition the reverse process of the diffusion model:

% \begin{equation}
% \epsilon_\theta(z_t, t, f_c) \approx \epsilon.
% \end{equation}

% This ensures that the generated images retain anatomically plausible structures, aligning with the individual patient's brain segmentation characteristics.


% Node Feature Reconstruction Loss  
% Each node feature \( v_i \) should be reconstructable from its learned embedding \( h_i \):

% \begin{equation}
% \mathcal{L}_{\text{node}} = \sum_{i=1}^{N} \left\| v_i - \hat{v}_i \right\|^2,
% \end{equation}

% where \( \hat{x}_i \) is the predicted feature from the graph embedding.

% Graph Structure Preservation Loss.
% To ensure the learned embeddings respect spatial relationships, we minimize the difference between the learned adjacency matrix \( A_{\text{pred}} \) and the original anatomical connectivity matrix \( A_{\text{true}} \):

% \begin{equation}
% \mathcal{L}_{\text{graph}} = \left\| A_{\text{pred}} - A_{\text{true}} \right\|^2.
% \end{equation}





% only a limited degree of control over the generated brain MRI 
%%%%  !!!!!!!!!!!!!!!
% it does not allow for conditioning the model on individual anatomical structures. 
% TODO
% The purpose of this block is to extend the capabilities of the LDM to encompass this additional control. To achieve this, we use ControlNet~\cite{zhang2023adding}, (block C in Figure~\ref{fig:pipeline}) a neural network designed to work in conjunction with the LDM. We conceptualize ControlNet and LDM as a unified network $\epsilon_{\theta,\phi}$, where $\theta$ represents the fixed network's parameters of the LDM and $\phi$ denotes the trainable network's parameters of ControlNet. As in the LDM, $\epsilon_{\theta,\phi}$ is still used to predict the noise $\epsilon_{\theta,\phi}(z_t, t, c, z)$ in the reverse diffusion step $z_t \to z_{t-1}$, now incorporating $z = \mathcal E(x)$ as a condition to encompass the structure of the target brain $x$ during the generation process. To train ControlNet, we use the latent representations $z^{(A)}$ and $z^{(B)}$ from pairs of brain MRIs of the same patient taken at different ages $A$ < $B$. The covariates $c^{(B)}$ associated with $z^{(B)}$ are known and used as target covariates. Each training iteration involves: i) sampling $t \sim U[1,T]$, ii) performing $t$ forward diffusion steps $z^{(B)} \to z_t^{(B)}$, iii) predicting the noise $\epsilon_{\theta,\phi}(z_t^{(B)}, t, c^{(B)}, z^{(A)})$ to revert $z^{(B)}_t \to z^{(B)}_{t-1}$, and iv) minimizing the loss $\mathcal{L}_{\epsilon}$ (Eq.~\ref{eqn:ddpmloss}).







% representation $z_0$




% applying the diffusion process to a latent representation $z_0$  rather than directly to the image  $x$ itself.

% The latent representation is obtained by training a pre-trained autoencoder, composed of an encoder $\mathcal{E}$ and a decoder $\mathcal{D},$ 






% In the forward process, Gaussian noise is incrementally added to the original image $x_0$ over $T$ steps. 




% This approach reduces the high memory demand while preserving the quality and flexibility of the models. 









% ------------------------



% vOur primary objective is to identify the commonalities among different views in the denoising process. To achieve this, we aim to discover the shared scene $z_x^k$ that is degradation-agnostic over various corrupted views $\{y_i^k\}_{k\in \mathbb N}$ via our proposed training schema, namely \textit{\textbf{M}ulti-view s\textbf{e}lf-supervised \textbf{D}isentanglement} (MeD). A graphic depiction of MeD is shown in Figure \ref{fig:arch}, composed of the representation learning process in the left panel, and four distinct reconstruction pathways in the right panel. 







% The progression in medical image synthesis domain, especially in langutudinal data 
% is much slower due the most of the existing datasets are relatively small-scale which may not be able to optimize the immense number of parameters of the generative model. ImageNet [5] plays an important role in various
% tasks in the image domain, but there is a lack of similar scale datasets in medical domain. 
% Therefore it is valuable if we can leverage the unlabeled data character to facilitate learning. Self-supervised learning
% is one kind of technique where the supervisory signal can be
% obtained easily from the data itself.





% This phrase is encoded by the text encoder and serves as the query input for the knowledge graph, which outputs local manifold editing for image feature tuning. The modified feature is then input into the pre-trained image decoder to synthesize the time-shifted longitudinal image. 

% After applying CLAP, the graph embodies the meaningful structure of longitudinal data. In this section, we will present the full framework of how our Graph As Control is used to synthesize 


% The learned graph encoder acts as a zero-shot structure learner by mapping image and description features into graph embeddings. 








\begin{figure}[htpb]
  % \hspace{-0.2pt}
  \centering
  \includegraphics[width=1.00 \linewidth ]{asset/img/arc.jpg}   % trim=5 110 20 10,clip
   \caption{Anatomical Geometry-Retrieval Graph.}
  \label{fig:graph}
\end{figure}




\subsection{Contrastive Longitudinal Alignment Prior}
\label{sec:clap}
Under interference posed by the posture noise, conventional supervision, i.e., pixel-wise loss function such as L1 and L2 which is unsuitable for this geometry-unpair supervision. Many before methods propose to use unpair loss, such as adversarial loss or style/perceptual loss, but this is more general to nature image which didn't consider the tight indentity consistency. 
 
As we dedicate to generate medical image in a geometry-sensitive way, we need to 
provide a new way that fit in medical domain that sensitive to petient indentity while perseving ability to indentify the longitudinal progression. 



With this goal, we presents \textit{Contrastive Longitudinal Alignment Prior}, denoted by CLAP, for effective satisfy the pre-assumed charateristic in medical domain. Under self-supervise manner, the CLAP is trained by complying the time-series nature of the longitudinal data and patient identity. In CLAP approach, we regulate each longitudinal set as a series of medical images from different patient $k1$ and $k2$, denoted as $\{x_t^{k1}\}_{t=1}^N$ and $\{x_t^{k2}\}_{t=1}^N$, corresponding to specified subscript time points indicated by $t$. 



% The subscript here indicates the longitudinal order. 


% Finally, the graph learning process is self-supervised by formulating an order alignment task. 
In this CLAP, images from $\{x_t^{k1}\}_{t=1}^N$ and $\{x_t^{k2}\}_{t=1}^N$ will be uniformly sampled and shuffled in a time manner to form the input data while the actual longitudinal order is served as the target, as shown in Fig. \ref{fig:clap}. To put it concere, assuming each patient sample $m$ longitudinal data, makes a $2m$ image set, them the image set got shuffled and put into the model to firstly do is to contrastively seperate longitudinal image of each patient in feature space. Then, in each seperation image set (patient-wise), the model reorder the shuffled longitudinal image in correct progression order to learn the progression process. 



% Assuming a tuple of 5 images, after graph generating and shuffle, we get $\langle g_1, G_4, G_3, G_2, G_5 \rangle$ with true order label $O=\langle 1, 4, 3, 2, 5 \rangle$. Then, the graphs are first pairwise concatenated $\mathbf{G}$ and transformed to form a tuple of five vectors capture the relationship between each graph with others. These vectors went throught a multi perceptron layer with linear activation for predicting the order. 


% Linear Distance
% The correctness of the prediction is measured using $\mathcal L_1$ distance:
% \begin{equation}
%     \mathcal{L}_1 = \sum^N_{n=1} |\hat y_n - y_n|
% \end{equation}

% where $\hat y_n$ and $y_n$ are the predicted order 
% mean squared error (MSE)


% Listwise approach to learning to rank: theory and algorithm
% ListMLE loss

The correctness of the order prediction is measured using ListMLE \cite{} loss:
\begin{equation}
\mathcal{L}_{\mathrm{MLE}}
% \left(\mathbf{p}_n\right)
=-\log \prod_{k=1}^{N} \frac{\exp \left(s_k\right)}{\sum_{i=k}^{N} \exp \left(s_i\right)},
\end{equation}

where $s$ represent the predicted scores sorted in descending order according to their corresponding order label in $O$. 



% Specifically, given any scene image $x^k \sim \mathcal{X}, k\in \mathbb N$ sampled uniformly from a clean image set $\mathcal{X}$, MeD produces two contaminated views:
% \begin{equation}
%     y_1^k \triangleq \mathcal{T}_1(x^k),\ 
%     y_2^k \triangleq \mathcal{T}_2(x^k),
% \end{equation}



while the $\mathcal{T}$ represent a random image geometry-transform operation, the CLAP is pre-trained between patients, given patient with $k1$ and $k2$, the longitudinal image sets of the are $\{x^{k1}_t\}_{t=1}^N, \{x^{k2}_t\}_{t=1}^N$, the CLAP evenly sample $m$ images from these two set with random timepoints, and combine them with shuffled order to create a new image set $\tilde X=\{\tilde x_1, \tilde x_2, \cdots, \tilde x_{2m}\}$. The CLAP then does two things of ordering longitudinal and sepeating patient indentity. 
\begin{equation}
 \hat{\text{I}}, \hat{\text{O}}  \triangleq \text{CLAP}(\tilde X),
\end{equation} 
where $ \hat{\text{I}}$ is indicating which patient the $x$ comes in, $k1$ or $k2$, to create a contrastive learn the difference between patient indentity. The $\hat{\text{O}}$ on the other hand, 

% 











\paragraph{Graph Structure of Image.}


% For each node $v_i$, we find its $K$ nearest neighbors $\mathcal{N}(v_i)$ and add an edge $e_{ji}$ directed from $v_j$ to $v_i$ for all $v_j\in\mathcal{N}(v_i)$. Then we obtain a graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$ where $\mathcal{E}$ denote all the edges. 


Which ViG block perform GraphConv~\cite{han2022vision}, given the input feature $X\in\mathbb{R}^{N\times D}$, the Grapher module can be expressed as:
\begin{equation}\label{eq:gcn}
	Y = \sigma(\text{GraphConv}(W_{in}X))W_{out} + X,
\end{equation}
where $Y\in\mathbb{R}^{N\times D}$, $W_{in}$ and $W_{out}$ are the weights of fully-connected layers, $\sigma$ is the activation function, \eg, GeLU~\cite{gelu}.  
To further encourage the feature transformation capacity and relief the over-smoothing phenomenon, we utilize feed-forward network (FFN) on each node. The FFN module is a simple multi-layer perceptron with two fully-connected layers:
\begin{equation}\label{eq:ffn}
	Z = \sigma(YW_{1})W_{2} + Y,
\end{equation}
where $Z\in\mathbb{R}^{N\times D}$, $W_{1}$ and $W_{2}$ are the weights of fully-connected layers, and the bias term is omitted. The hidden dimension of FFN is usually larger than $D$. In both Grapher and FFN modules, batch normalization is applied after every fully-connected layer or graph convolution layer, which is omitted in Eq.~\ref{eq:gcn} and \ref{eq:ffn} for concision.
To train the Vision Graph Network, we employ a contrastive learning objective that enforces structural consistency by mapping similar segmentation patterns to proximate embeddings while preserving geometric relationships. The graph representation loss is defined by key components, including contrastive loss for patient-specific features.

To ensure that segmentation maps of anatomically similar patients yield comparable embeddings while maintaining distinctiveness across individuals, we optimize the following contrastive loss:

\begin{equation}
\mathcal{L}_{\text{cont}} = \sum_{(i,j) \in \mathcal{P}} d(h_i, h_j) - \sum_{(i,k) \in \mathcal{N}} \max(0, m - d(h_i, h_k)).
\end{equation}

where \( d(h_i, h_j) \) measures the distance between embeddings, \( \mathcal{P} \) represents positive pairs (patients with similar segmentation maps), and \( \mathcal{N} \) denotes negative pairs (distinct patients). The margin \( m \) mitigates collapsed embeddings by enforcing sufficient separation.  


After training, the Vision Graph Network produces a patient-specific geometric feature vector, formulated as node-level output $f_c = \mathcal{V}$,  which serves as a conditioning signal for the diffusion model, guiding the generative process to preserve patient-specific anatomical structures.





\paragraph{Reformed Generation Process}
% While diffusion model can generate high fedality image, it didn't meet the requriement of medical image as 
In this paper, we reform the generation process by aligning anatomical geometry-retrival graph $g_t^k$ in the generation process as geometery prior. As illustrated in Fig. \ref{fig:clap}, 
our \textit{Anatomical Geometry-Retrieval Graph} is constructed upon key structure segmentations as graph nodes, which allows us to accurately represent and analyze the complex relationships between different anatomical structures and functional topography.



Given a image $x_t^k$ at specific timestamp $t$, we desire the model generate longitudinal images at desired timestamp $t+d$, with a condition query phrase $c_d$ for the desired timestamp, such as “How is this patient in $d$ months later?”.  Then let the generator does the following process:
\begin{equation}
   \hat x_{t+d}^k \triangleq \mathit{F}_\theta(x^k_t, g^k_t;\ c_d),
\end{equation} 





